A minimalistic approach for fast computation of geodesic distances on triangular meshes

The computation of geodesic distances is an important research topic in Geometry Processing and 3D Shape Analysis as it is a basic component of many methods used in these areas. In this work, we present a minimalistic parallel algorithm based on front propagation to compute approximate geodesic distances on meshes. Our method is practical and simple to implement and does not require any heavy pre-processing. The convergence of our algorithm depends on the number of discrete level sets around the source points from which distance information propagates. To appropriately implement our method on GPUs taking into account memory coalescence problems, we take advantage of a graph representation based on a breadth-first search traversal that works harmoniously with our parallel front propagation approach. We report experiments that show how our method scales with the size of the problem. We compare the mean error and processing time obtained by our method with such measures computed using other methods. Our method produces results in competitive times with almost the same accuracy, especially for large meshes. We also demonstrate its use for solving two classical geometry processing problems: the regular sampling problem and the Voronoi tessellation on meshes.

==> algorithms/farthest_point_sampling.tex <==
\begin{algorithmic}[1]
    \REQUIRE Triangular mesh $(V,F)$, source vertex $s \in V$, number of samples $m$
    \ENSURE Sampling vertices set $S \subset V$
	\STATE $S \Leftarrow \{s\}$
	\WHILE{$|S| < m$}
		\STATE $d \Leftarrow $ \textbf{compute\_geodesics$(V, F, S)$}\label{alg:fps:distances}
		\STATE $s \Leftarrow \displaystyle\arg\max_{v \in V} d(v)$
		\STATE $S \Leftarrow S \cup \{s\}$
	\ENDWHILE
	\RETURN $S$
\end{algorithmic}


==> algorithms/fastmarching.tex <==
\begin{algorithmic}[1]
    \REQUIRE Triangular mesh $(V, F)$, source vertices $S \subset V$
    \ENSURE Distances map $d : V \rightarrow \mathbb{R}$
	\STATE $\forall v \in V : d(v) \Leftarrow \infty$, $\forall s \in S : d(s) \Leftarrow 0$
	\STATE $R \Leftarrow S$
	\STATE $G \Leftarrow V \setminus R$
	\STATE $B \Leftarrow \{\}$
	\WHILE{$B \not = V$}
		\STATE $v \Leftarrow \displaystyle\arg\min_{v \in R} d(v)$
		\STATE $R \Leftarrow R \setminus \{v\}$
		\STATE $B \Leftarrow B \cup \{v\}$
		\FORALL{$v_0 \in \mathcal{N}(v)$}
			\STATE $G \Leftarrow G \setminus \{v_0\}$
			\STATE $R \Leftarrow R \cup \{v_0\}$
			\FORALL{$(v_0, v_1, v_2) \in F(v_0)$}
				\STATE $d(v_0) \Leftarrow \min\{d(v_0)$, \hyperref[algorithms/planar_update]{\textit{update\_step}$(d_{k-1}, v_0, v_1, v_2)$}$\}$
			\ENDFOR
		\ENDFOR
	\ENDWHILE
	\RETURN $d$
\end{algorithmic}


==> algorithms/planar_update.tex <==
\begin{algorithmic}[1]
    \REQUIRE A distance map $d:V \rightarrow \mathbb{R}$, triangular face $(v_0, v_1, v_2) \in F$.
    \ENSURE Solution of the Eikonal equation for the triangle $(v_0, v_1, v_2)$ and the vertex $v_0$.
	\STATE $x_1 \Leftarrow v_1 - v_0$
	\STATE $x_2 \Leftarrow v_2 - v_0$
	\STATE $X \Leftarrow \begin{bmatrix} x_1 & x_2 \end{bmatrix} $
	\STATE $t \Leftarrow \begin{bmatrix} d(v_1) & d(v_2)\end{bmatrix}^T$
	\STATE $1^T = \begin{bmatrix} 1 & 1 \end{bmatrix}$
	\STATE $p \Leftarrow \displaystyle\frac{1^TQt + \sqrt{(1^TQt)^2 - 1^TQ1 \cdot (t^TQt - 1)}}{1^TQ1}$
	\STATE $n \Leftarrow XQ(t - 1)$
	\IF{$QX^Tn < 0$}
		\RETURN $p$
	\ELSE	
		\RETURN $\min\{d_{k - 1}(v_1) + \|x_1\|, d_{k - 1}(v_2) + \|x_2\|\}$
	\ENDIF
\end{algorithmic}


==> algorithms/ptp.tex <==
\begin{algorithmic}[1]
    \REQUIRE Triangular mesh $(V,F)$, source vertices $S \subset V$
    \ENSURE Distances map $d : V \rightarrow \mathbb{R}$
	
	\STATE $d_k$ current distance map at iteration $k$
%	\STATE Compute \toplesets $V_r$, $\forall r \in [0,\rho]$
	
	\STATE $\forall v \in V : d_0(v) \Leftarrow \infty$
	\STATE $\forall s \in S : d_0(s) \Leftarrow 0$
	
	\STATE $i \Leftarrow 1$, $j \Leftarrow 1$, $k \Leftarrow 1$
	
	\WHILE{$i \leq j$}
		\FORALL{$v_0 \in \displaystyle\bigcup_{r = i}^{j} V_r$ \textbf{\color{blue!64}(in parallel)}}\label{alg:ptp_iter_line}
			\STATE $d_k(v_0) \Leftarrow d_{k-1}(v_0)$
			\FORALL{$(v_0, v_1, v_2) \in F(v_0)$}
				\STATE $d_k(v_0) \Leftarrow \min\{d_k(v_0)$, \hyperref[algorithms/planar_update]{\textit{update\_step}$(d_{k-1}, v_0, v_1, v_2)$}$\}$
			\ENDFOR
		\ENDFOR

		\IF{$\displaystyle\frac{\left|d_k(v) - d_{k-1}(v)\right|}{d_{k-1}(v)} < \epsilon, \forall v \in V_i$}
			\STATE $i \Leftarrow i + 1$
		\ENDIF

		\STATE $ k \Leftarrow k + 1$

		\IF{$k < \rho$}
			\STATE $j \Leftarrow k$
		\ENDIF

	\ENDWHILE

	\RETURN $d \Leftarrow d_K$
\end{algorithmic}



==> algorithms/ptp_fixed_band.tex <==
\begin{algorithmic}[1]
    \REQUIRE Triangular mesh $(V,F)$, source vertices $S \subset V$, $V_r$ and $r \in [0, \rho]$
    \ENSURE Distances map $d : V \rightarrow \mathbb{R}$
	\STATE pre-compute $s(B(k))$ for each $k$-topleset
	\STATE $d_k$ current distance map at iteration $k$
	\STATE $\forall v \in V : d_0(v) \Leftarrow \infty$
	\STATE $\forall s \in S : d_0(s) \Leftarrow 0$
	\STATE $d_1 \Leftarrow d_0$
	\FOR{$k \Leftarrow 1$ to $K$}
		\FORALL{$v_0 \in \bigcup_{r = s(B(k))}^{k} V_r$ \textbf{\color{blue!64}(in parallel)}}\label{alg:fastmarching_approach_iter_line}
			\FORALL{$(v_0, v_1, v_2) \in F(v_0)$}
				\STATE \hyperref[alg:update-n]{update$(d_k, d_{k-1}, v_0, v_1, v_2)$}
			\ENDFOR
		\ENDFOR
	\ENDFOR
	\RETURN $d \Leftarrow d_K$
\end{algorithmic}


==> figures/deg_meshes.tex <==
\centering
\foreach \filename in \meshes
{
	\subcaptionbox{\em \StrSubstitute{\filename}{_}{\_} }
	{\includegraphics[width = 0.19\linewidth]{figures/deg_\filename}}
}



==> figures/fps_times_sources.tex <==
\centering
\foreach \filename in \meshes
{
	\subcaptionbox{\em \StrSubstitute{\filename}{_}{\_} }
	{\includegraphics[width = 0.48\linewidth]{figures/fps_times_\filename}}
}



==> figures/ptp_band_toplesets.tex <==
\centering
\foreach \filename in \meshes
{
	\subcaptionbox{\em \StrSubstitute{\filename}{_}{\_} }
	{\includegraphics[width = 0.19\linewidth]{figures/ptp_band_toplesets_\filename}}
}



==> figures/ptp_band_vertices.tex <==
\centering
\foreach \filename in \meshes
{
	\subcaptionbox{\em \StrSubstitute{\filename}{_}{\_} }
	{\includegraphics[width = 0.19\linewidth]{figures/ptp_band_vertices_\filename}}
}



==> figures/ptp_iter_error.tex <==
\centering
\foreach \filename in \meshes
{
	\subcaptionbox{\em \StrSubstitute{\filename}{_}{\_} }
	{\includegraphics[width = 0.19\linewidth]{figures/ptp_iter_error_\filename}}
}



==> figures/ptp_iter_error_double.tex <==
\centering
\foreach \filename in \meshes
{
	\subcaptionbox{\em \StrSubstitute{\filename}{_}{\_} }
	{\includegraphics[width = 0.19\linewidth]{figures/ptp_iter_error_double_\filename}}
}



==> figures/ptp_meshes.tex <==
\centering
\foreach \filename in \meshes
{
	\subcaptionbox{\em \StrSubstitute{\filename}{_}{\_} }
	{\includegraphics[width = 0.1\linewidth]{figures/ptp_\filename}}
}



==> figures/ptp_times_sources.tex <==
\centering
\foreach \filename in \meshes
{
	\subcaptionbox{\em \StrSubstitute{\filename}{_}{\_} }
	{\includegraphics[width = 0.48\linewidth]{figures/ptp_times_\filename}}
}



==> figures/toplesets_meshes.tex <==
\centering
\foreach \filename in \meshes
{
	\subcaptionbox{\em \StrSubstitute{\filename}{_}{\_} }
	{\includegraphics[width = 0.19\linewidth]{figures/\filename_toplesets}}
}



==> figures/toplesets_sorted_meshes.tex <==
\centering
\foreach \filename in \meshes
{
	\subcaptionbox{\em \StrSubstitute{\filename}{_}{\_} }
	{\includegraphics[width = 0.19\linewidth]{figures/\filename_toplesets_sorted}}
}



==> sections/abstract_old.tex <==
\begin{abstract}

The computation of geodesic distances is an important research topic in Geometry Processing and
3D Shape Analysis as it is a basic component of many methods used in these areas. For this reason,
different approaches have been proposed to compute geodesic distances including exact and 
approximate methods. Approximate methods are usually used when efficiency is mandatory and
particularly when dealing with large meshes. One of the most well-known methods used for computing
approximate geodesic distances is the Fast Marching algorithm. Recently, new methods have been
proposed: the spectral and diffusion flow-based methods. These approaches are very efficient for
distance query but usually depend on computationally intensive preprocessing steps. In this work,
we present an iterative parallel algorithm based on front propagation to compute approximate
geodesic distances on meshes that is practical and simple to implement. The convergence of our
iterative algorithm depends on the number of discrete level sets around the source points from which
distance information propagates. To appropriately implement our method on GPUs taking into account
memory coalescence problems, \textcolor{red}{we devised a new graph representation} based on a breadth-first search
traversal that works harmoniously with our parallel front propagation approach. In the experiments,
we show how our method scales with the size of the problem by using the \textcolor{red}{proposed graph representation}. 
We compare its mean error and processing times with such measures computed using other methods. We
also demonstrate its use for solving two classical geometry processing problems: the regular sampling
problem and the Voronoi tessellation on meshes.


%-------------------------------------------------------------------------
%  ACM CCS 1998
%  (see http://www.acm.org/about/class/1998)
% \begin{classification} % according to http:http://www.acm.org/about/class/1998
% \CCScat{Computer Graphics}{I.3.3}{Picture/Image Generation}{Line and curve generation}
% \end{classification}
%-------------------------------------------------------------------------
%  ACM CCS 2012
%   (see http://www.acm.org/about/class/class/2012)
%The tool at \url{http://dl.acm.org/ccs.cfm} can be used to generate
% CCS codes.
%Example:

\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003752.10003809.10010170</concept_id>
<concept_desc>Theory of computation~Parallel algorithms</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10003752.10010061.10010063</concept_id>
<concept_desc>Theory of computation~Computational geometry</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010371.10010396.10010397</concept_id>
<concept_desc>Computing methodologies~Mesh models</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010371.10010396.10010398</concept_id>
<concept_desc>Computing methodologies~Mesh geometry models</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010371.10010396.10010402</concept_id>
<concept_desc>Computing methodologies~Shape analysis</concept_desc>
<concept_significance>300</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[300]{Theory of computation~Parallel algorithms}
\ccsdesc[300]{Theory of computation~Computational geometry}
\ccsdesc[300]{Computing methodologies~Mesh models}
\ccsdesc[300]{Computing methodologies~Mesh geometry models}
\ccsdesc[300]{Computing methodologies~Shape analysis}

\printccsdesc
\end{abstract}



==> tables/complexity.tex <==
\begin{tabular}{|l|c|}	\hline
\textbf{Algorithm}																											& \textbf{Complexity}								\\\hline
\hyperref[algorithms/planar_update]{Update Fast Marching}												
					& $ O(1) $											\\\hline
\hyperref[algorithms/fastmarching]{Fast Marching}														
					& $ O(n \log n) $									\\\hline	
\hyperref[algorithms/farthest_point_sampling]{Farthest Point Sampling}									
					& $ O(m n \log n) $									\\\hline	
\hyperref[algorithms/planar_update_approach]{Update Fast Marching modified}							
						& $ O(1) $											\\\hline	
\hyperref[algorithms/fastmarching_approach]{\appname{}}												
						& $ O\left(\sqrt{\frac{n}{m}}\frac{n}{\mathcal{T}}\right) $	\\\hline
\hyperref[algorithms/farthest_point_sampling]{Farthest Point Sampling} with 
\hyperref[algorithms/fastmarching_approach]{\appabrv}			
& $ 
O\left(\sqrt{m}\frac{n^{3/2}}{\mathcal{T}}\right) $		\\\hline		
\end{tabular}


==> tables/fm_tests.tex <==
% single precision
\resizebox{\linewidth}{!}{%
	\begin{tabular}{|rr|rr|rr|} \hline
%
	\rowcolor{gray!40}  
	\multicolumn{2}{|r|}{\textbf{double precision}}		&
	\multicolumn{2}{c|}{\textbf{FM toolbox}}			&
	\multicolumn{2}{c|}{\textbf{FM ours}}				\\
%
	\rowcolor{gray!40}  
	\textsc{Filename}						&
	\textsc{Vertices}						&
	\textsc{Time}							&
	\textsc{Error}							&
	\textsc{Time}							&
	\textsc{Error}							\\
%
	\hline
	\rowcolor{white}  
	\input{tests/fm_results}
	\hline
	\end{tabular}
}



==> tables/ptp_tests.tex <==
% single precision
\resizebox{0.75\textwidth}{!}{%
	\begin{tabular}{|rr|rr|r>{\color{blue!64}}rr|r>{\color{blue!64}}rr|} \hline
%
	\rowcolor{gray!40}  
	\multicolumn{2}{|r|}{\textbf{single precision}}		&
	\multicolumn{2}{c|}{\textsc{Fast Marching}}			&
	\multicolumn{3}{c|}{\textbf{\appabrv~ (OpenMP)}}	&
	\multicolumn{3}{c|}{\textbf{\appabrv~ (cuda)}}	 	\\
%
	\rowcolor{gray!40}  
	\textsc{Filename}						&
	\textsc{Vertices}						&
	\textsc{Time}							&
	\textsc{Error}							&
	\multicolumn{2}{c}{\textsc{Time}}		&
	\textsc{Error}							&
	\multicolumn{2}{c}{\textsc{Time}}		&
	\textsc{Error}							\\
%
	\hline
	\rowcolor{white}  
	\input{tests/ptp_results}
	\hline
	\end{tabular}
}



==> tables/ptp_tests_double.tex <==
	% double precision
\resizebox{0.95\textwidth}{!}{%
	\rowcolors{2}{white}{gray!15} 
	\begin{tabular}{|rr|rr|r>{\color{blue!64}}rrl|>{\color{orange}}rr>{\color{blue!64}}rrl|} \hline
%	
	\rowcolor{gray!40}  
	\multicolumn{2}{|r|}{\textbf{double precision}}					&
	\multicolumn{2}{c|}{\textsc{Fast Marching}}						&
	\multicolumn{4}{c|}{\textbf{\appabrv~ (OpenMP / cuda)}}			&
	\multicolumn{5}{c|}{\textsc{Heat Method} (Cholmod / cusolverSp)}	\\
%
	\rowcolor{gray!40}  
	\textsc{Filename}						&
	\textsc{Vertices}						&
	\textsc{Time}							&
	\textsc{Error}							&
	\multicolumn{2}{c}{\textsc{Time}}		&
	\textsc{Error}							&&
	\textsc{Precomp}						&
	\multicolumn{2}{c}{\textsc{Solve}}		&
	\textsc{Error}							&\\
%
	\hline
	\input{tests/ptp_results_double}
	\end{tabular}
}



==> tests/fm_results.tex <==
      \verb|fandisk| &         6475 &    \bf  0.053s & \bf 0.95\%		& 0.105s		& 1.07\%\\
\verb|bunny_irregular| &       7500 &    \bf  0.078s & \bf 1.49\%		& 0.129s		& 2.14\%\\
       \verb|kitten| &        14472 &    \bf  0.138s & \bf 1.13\%		& 0.232s		& 1.13\%\\
     \verb|elephant| &        24955 &    \bf  0.323s & \bf 0.88\%		& 0.403s		& 0.90\%\\
        \verb|bunny| &        34835 &    \bf  0.497s & \bf 0.91\%		& 0.558s		& 0.96\%\\
         \verb|tyra| &       100002 &         1.991s & \bf 0.77\%		& \bf 1.665s		& 0.93\%\\
    \verb|armadillo| &       172974 &         4.395s & \bf 0.62\%		& \bf 2.838s		& 0.73\%\\
     \verb|ramesses| &       826266 &        24.769s & \bf 0.54\%		& \bf 13.838s		& 0.64\%\\
       \verb|dragon| &      3609455 &       733.167s & \bf 0.37\%		& \bf 56.988s		& 0.39\%\\



==> tests/ptp_results.tex <==
      \verb|fandisk| &         6475 &         0.158s &    \bf  1.07\% &    \bf  0.006s & \bf (25.3x) &         1.07\% &         0.008s & \bf (19.2x) &         1.07\% \\
\verb|bunny_irregular| &         7500 &         0.195s &         2.14\% &    \bf  0.008s & \bf (23.0x) &    \bf  2.12\% &         0.010s & \bf (18.9x) &         2.12\% \\
       \verb|kitten| &        14472 &         0.357s &    \bf  1.13\% &    \bf  0.009s & \bf (38.9x) &         1.14\% &         0.012s & \bf (30.4x) &         1.14\% \\
     \verb|elephant| &        24955 &         0.624s &    \bf  0.90\% &         0.018s & \bf (34.3x) &         0.91\% &    \bf  0.015s & \bf (40.7x) &         0.91\% \\
        \verb|bunny| &        34835 &         0.864s &    \bf  0.96\% &         0.024s & \bf (36.7x) &         0.96\% &    \bf  0.015s & \bf (57.0x) &         0.96\% \\
         \verb|tyra| &       100002 &         2.571s &    \bf  0.93\% &         0.137s & \bf (18.7x) &         1.00\% &    \bf  0.032s & \bf (79.5x) &         1.01\% \\
    \verb|armadillo| &       172974 &         4.391s &    \bf  0.72\% &         0.121s & \bf (36.2x) &         0.89\% &    \bf  0.035s & \bf (126.7x) &         0.90\% \\
     \verb|ramesses| &       826266 &        21.438s &    \bf  0.51\% &         1.978s & \bf (10.8x) &         1.28\% &    \bf  0.263s & \bf (81.6x) &         1.35\% \\
       \verb|dragon| &      3609455 &        89.149s &         0.28\% &        10.946s & \bf (8.1x) &    \bf  0.27\% &    \bf  1.732s & \bf (51.5x) &         0.31\% \\


==> tests/ptp_results_double.tex <==
      \verb|fandisk| &         6475 &         0.159s &         1.07\% &         0.005s & \bf (29.4x) &         1.07\% & OpenMP &  0.068s &    \bf  0.002s & \bf (101.1x) &         0.84\% & Cholmod \\
&&& &         0.009s & \bf (18.6x) &         1.07\% & Cuda &  0.855s &         0.646s & \bf (0.2x) &    \bf  0.84\% & cusolverSp \\\hline
\verb|bunny_irregular| &         7500 &         0.195s &         2.14\% &         0.008s & \bf (24.6x) &    \bf  2.12\% & OpenMP &  0.085s &    \bf  0.002s & \bf (117.1x) &        14.28\% & Cholmod \\
&&& &         0.011s & \bf (18.3x) &         2.12\% & Cuda &  0.862s &         1.225s & \bf (0.2x) &        14.28\% & cusolverSp \\\hline
       \verb|kitten| &        14472 &         0.357s &    \bf  1.13\% &         0.009s & \bf (41.1x) &         1.14\% & OpenMP &  0.189s &    \bf  0.004s & \bf (96.9x) &         1.29\% & Cholmod \\
&&& &         0.012s & \bf (29.6x) &         1.14\% & Cuda &  0.888s &         1.235s & \bf (0.3x) &         1.29\% & cusolverSp \\\hline
     \verb|elephant| &        24955 &         0.623s &    \bf  0.90\% &         0.017s & \bf (36.0x) &         0.91\% & OpenMP &  0.307s &    \bf  0.006s & \bf (102.3x) &         0.99\% & Cholmod \\
&&& &         0.016s & \bf (39.4x) &         0.91\% & Cuda &  0.902s &         1.733s & \bf (0.4x) &         0.99\% & cusolverSp \\\hline
        \verb|bunny| &        34835 &         0.863s &         0.96\% &         0.023s & \bf (37.3x) &         0.97\% & OpenMP &  0.444s &    \bf  0.009s & \bf (95.7x) &    \bf  0.93\% & Cholmod \\
	&&& &         0.016s & \bf (52.8x) &         0.97\% & Cuda &  0.953s &        20.694s & \bf (0.0x) &         0.93\% & cusolverSp \\\hline
         \verb|tyra| &       100002 &         2.572s &    \bf  0.93\% &         0.139s & \bf (18.5x) &         1.02\% & OpenMP &  1.340s &    \bf  0.029s & \bf (89.4x) &         1.16\% & Cholmod \\
&&& &         0.036s & \bf (71.2x) &         1.02\% & Cuda &    infs &           infs & \bf (0.0x) &           inf\% & cusolverSp \\\hline
    \verb|armadillo| &       172974 &         4.390s &         0.72\% &         0.122s & \bf (36.0x) &         0.90\% & OpenMP &  2.384s &         0.066s & \bf (66.8x) &    \bf  0.59\% & Cholmod \\
&&& &    \bf  0.038s & \bf (114.3x) &         0.90\% & Cuda &    infs &           infs & \bf (0.0x) &           inf\% & cusolverSp \\\hline
     \verb|ramesses| &       826266 &        21.449s &    \bf  0.64\% &         1.678s & \bf (12.8x) &         1.89\% & OpenMP & 12.067s &         0.347s & \bf (61.7x) &           nan\% & Cholmod \\
&&& &    \bf  0.268s & \bf (80.2x) &         1.89\% & Cuda &    infs &           infs & \bf (0.0x) &           inf\% & cusolverSp \\\hline
       \verb|dragon| &      3609455 &        89.054s &    \bf  0.39\% &         9.311s & \bf (9.6x) &         0.68\% & OpenMP & 60.709s &         2.628s & \bf (33.9x) &           nan\% & Cholmod \\
&&& &    \bf  1.596s & \bf (55.8x) &         0.68\% & Cuda &    infs &           infs & \bf (0.0x) &           inf\% & cusolverSp \\\hline

